Vidi2.5: Large Multimodal Models for Video Understanding and Creation

Video has emerged as the primary medium for communication and creativity on the Internet, driving strong demand for scalable, high-quality video production. Vidi models continue to evolve toward next-generation video creation and have achieved state-of-the-art performance in multimodal temporal retrieval (TR). In its second release, Vidi2 advances video understanding with fine-grained spatio-temporal grounding (STG) and extends its capability to video question answering (Video QA), enabling comprehensive multimodal reasoning. Given a text query, Vidi2 can identify not only the corresponding timestamps but also the bounding boxes of target objects within the output time ranges. To enable comprehensive evaluation of STG, we introduce a new benchmark, VUE-STG, which offers critical improvements over existing STG datasets. In addition, we upgrade the previous VUE-TR benchmark to VUE-TR-V2, achieving a more balanced duration and query distribution. Remarkably, the Vidi2 model substantially outperforms leading proprietary systems, such as Gemini 3 Pro Preview and GPT-5, on both VUE-TR-V2 and VUE-STG, while achieving competitive results with popular open-source models with similar scale on video QA benchmarks. The latest Vidi2.5 offers significantly stronger STG capability and slightly better TR and Video QA performance over Vidi2. This update also introduces a Vidi2.5-Think model to handle plot understanding with complex plot reasoning. To comprehensively evaluate the performance of plot understanding, we propose VUE-PLOT benchmark with two tracks, Character and Reasoning. Notably, Vidi2.5-Think outperforms Gemini 3 Pro Preview on fine-grained character understanding with comparable performance on complex plot reasoning. Furthermore, we demonstrate the effectiveness of Vidi2.5 on a challenging real-world application, video editing planning.

==> sections/app_fg.tex <==
\section{Applications: Semantic-Driven Video Orchestration}
\label{sec:applications}

In this work, we showcase an agentic application of \methodnew{}, specifically \textbf{\textit{semantic-driven video orchestration}}. Unlike traditional tasks that end at perception, this application requires the model to act as an autonomous agent capable of synthesizing raw assets into a coherent product. Through our qualitative results, we highlight the agentic capabilities of \methodnew{} in three key dimensions:

\begin{itemize}
    \item \textbf{Material Comprehension \& Insight:} The ability to ground semantic concepts within raw, uncurated video observations and extract high-level distinct features necessary for storytelling.
    \item \textbf{Narrative Architecture \& Planning:} The capacity for long-horizon reasoning, enabling the model to organize disjoint clips into a logical temporal structure with a coherent narrative arc.
    \item \textbf{Structured Assembly \& Refinement:} The proficiency to translate abstract intents into rigorous, structured specifications that guide downstream execution tools.
\end{itemize}


\subsection{Semantic-Driven Video Orchestration as Agentic Reasoning}

Video editing planning is framed here as a complex planning task where an agent must determine a set of interdependent decisions to compose a final video from a pool of raw observations. Given a collection of source clips and a high-level user intent, the objective is to generate an \textit{editing plan}—a symbolic representation acting as a blueprint for narrative structure, audio-visual alignment, and stylistic execution.

{\flushleft Crucially, the editing plan serves as a unified intermediate representation that bridges the gap between the agent's semantic reasoning and the low-level rendering system. It encapsulates the agent's "thought process" regarding how the final output should be realized.}

\subsection{Editing Plan Specification: The Action Space}

At the planning level, the editing plan defines the agent's action space. As illustrated in Figure~\ref{fig:application_planner}, these decisions are not merely descriptive but are semantic specifications for downstream execution.

\paragraph{Narrative Structure (Temporal Reasoning):} This component represents the agent's core planning capability—orchestrating the temporal backbone of the video. It involves selecting relevant segments from raw footage and ordering them to construct a logical flow (e.g., chronological, causal, or thematic), governing how visual content conveys the intended story.

\paragraph{Voiceover Content (Multimodal Alignment):} The specification of spoken content that aligns with the visual narrative. The agent generates the script, delivery style, and precise temporal alignment, ensuring that the narration complements rather than competes with the visual progression.

\paragraph{Audio Attributes (Atmospheric Design):} The characterization of auditory elements, such as music genre, mood, and rhythmic profile. This establishes the auditory framing, promoting coherence between the soundscape and the visual pacing.

\paragraph{Visual Editing Intent (Stylistic Directives):} The articulation of transition designs, emphasis cues, and visual effects in semantic terms. This translates the agent's "director's cut" intuition into actionable instructions for the rendering engine.

{\flushleft Together, these categories define a structured output space, allowing the agent to express complex editing logic while remaining agnostic to the specific implementation details of the rendering software.}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[height=0.9\textheight, keepaspectratio]{sections/figures/application_planner.pdf}
    \caption{Overview of the \vidiedit{} execution pipeline. The VLM acts as a high-level planner, generating a structured editing plan that specifies narrative structure, voiceover content, audio attributes, and visual editing directives. This plan is subsequently translated into concrete operations (audio synthesis, effect application, rendering) by the execution engine.}
    \label{fig:application_planner}
\end{figure*}

\subsection{Post-Training for Planning Alignment}

To transition from a general-purpose VLM to a specialized planning agent, we post-train \methodnew{} to align its reasoning capabilities with the rigid requirements of editing plan generation. We refer to this configuration as \vidiedit{}. 

{\flushleft This stage focuses on \textit{output structuring} and \textit{semantic consistency}. We utilize task-specific supervision where inputs are paired with structured editing plans (e.g., JSON-formatted sequences). The training objective emphasizes adherence to the schema and logical coherence across modalities, enabling the model to reliably output parsable, execution-ready plans rather than unstructured free text.}

\subsection{Plan Execution: From Intent to Realization}

The editing plans generated by \vidiedit{} are designed to be consumed by an execution pipeline. As illustrated in Figure~\ref{fig:application_planner}, \fg{this pipeline acts as the ``tool" invoked by the agent, translating high-level semantic specifications into low-level media operations. (I intentionally overclaim this part to emphasize the agent tool use capability)}

{\flushleft Concretely, realization proceeds by instantiating the semantics specified in the editing plan. Audio assets, including background music and narration voices, are selected via retrieval from curated databases according to the plan’s audio attributes. Visual editing intent is further translated into executable effect parameters, which are applied during video rendering to produce the edited video. An in-house rendering system integrates video and audio streams, overlays generated text, and applies visual effects to synthesize the final output.}

\subsection{Qualitative Analysis}

We examine the editing plans produced by \vidiedit{} to illustrate how high-level agentic intent is reflected in the final outputs. Figures~\ref{fig:application_planner_cats2}--\ref{fig:application_planner_mix2} display representative frames that visualize the agent's decisions regarding clip arrangement and narrative progression.

{\flushleft The results demonstrate that \vidiedit{} produces coherent plans that impose an explicit temporal structure on raw inputs. The ordering reflects a planned narrative arc—establishing context, developing the core message, and concluding effectively. Furthermore, the generated voiceover demonstrates strong alignment with visual changes, suggesting that the model maintains a synchronized internal state of both visual and textual modalities during the planning process.}

{\flushleft While the figures visualize the visual sequence, the holistic quality of the agent's planning (including audio-visual synergy) is best appreciated through dynamic playback. Additional video examples and an interactive demo of the system are available on the project website.}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[height=0.9\textheight, keepaspectratio]{sections/figures/application_planner_cats2.pdf}
    \caption{Qualitative example of an editing plan generated by \vidiedit{} for a single-topic scenario. The model successfully identifies key moments and arranges them to support a cohesive narrative.}
    \label{fig:application_planner_cats2}
\end{figure*}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[height=0.9\textheight, keepaspectratio]{sections/figures/application_planner_mix2.pdf}
    \caption{Qualitative example of an editing plan generated by \vidiedit{} for a mixed-content scenario, demonstrating the agent's ability to synthesize disparate raw clips into a unified storyline.}
    \label{fig:application_planner_mix2}
\end{figure*}

==> sections/figures/plot_performance_v3.tex <==
\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l| l| c | c c c c c}
\toprule[1.2pt]
\multirow{2}{*}{Track} & \multirow{2}{*}{Category} & \multirow{2}{*}{Metric(\%)} 
& \multicolumn{5}{c}{Models} \\
\cline{4-8}
~ & ~ & ~ 
& \shortstack{\textbf{Vidi}\\\textbf{2.5}}
& \shortstack{Gemini\\3 Pro}
& \shortstack{GPT\\5}
& \shortstack{Qwen3\\VL}
& \shortstack{Qwen3\\Omni} \\
\hline

\multirow{3}{*}{Char.} & \multirow{3}{*}{-} 
~ & tIoU & \textbf{71.63} & 66.04 & - & - & 50.68 \\
~ & ~ & sIoU & \textbf{55.89} & 13.24 & - & - & 6.80 \\
~ & ~ & WER $\downarrow$ & \textbf{23.20} & 29.00 & - & - & 58.12 \\

\hline\hline
\multirow{5}{*}{Rea.} 
~ & Perception and Understanding & Acc  & 66.25 & \textbf{80.42} & 55.83 & 35.00 & 40.83 \\
~ & Speech, Audio, and Sound Effect Reasoning & Acc & \textbf{74.43} & 66.03 & 55.34 & 45.42 & 27.10 \\
~ & Social Cognition and Knowledge Integration & Acc & \textbf{62.78} & 62.15 & 53.94 & 31.23 & 23.03 \\
~ & Narrative and Structural Understanding & Acc & 55.17 & \textbf{59.48} & 51.72 & 25.86 & 25.00 \\
~ & Professional Filming and Editing Techniques & Acc & \textbf{61.35} & 50.92 & 55.21 & 30.67 & 24.54 \\
\hline
~ & Overall & Acc & 64.33 & \textbf{64.58} & 54.37 & 33.94 & 28.01 \\
\bottomrule[1.2pt]
\end{tabular}}
\caption{
Evaluation results on the VUE-CHAR benchmark, reporting temporal intersection-over-union (tIoU), spatial intersection-over-union (sIoU) and ASR errors in the \textit{Character} (Char.) and question accuracy in the \textit{Reasoning} (Rea.) track.\zf{Update }}
\label{tab:plot_results_t}
\end{table}


==> sections/tables/plot_performance.tex <==
\begin{table}[!htbp]
\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{l| l c | c c c c c}
\toprule[1.2pt]
Major Type & Category & Metric(\%) & \textbf{Vidi2.5} & Gemini 3 Pro. & GPT-5  & Qwen3-VL & Qwen3-Omni \\
\hline

\multirow{3}{*}{Character} & \multirow{3}{*}{-} 
~ &   tIoU & \textbf{71.74} & 66.04 & - & - & 49.31 \\
~ & ~ & sIoU & \textbf{60.31} & 12.99 & - & - & 7.74 \\
~ & ~ & WER $\downarrow$ & \textbf{23.15} & 28.20 & - & - & 56.36 \\

\hline\hline
\multirow{5}{*}{Reasoning} 
~& Perception and Understanding & Acc  & 66.25 & \textbf{80.42} & - & 35.00 & 40.83 \\
~& Speech, Audio, and Sound Effect Reasoning & Acc & \textbf{74.43} & 66.03 & - & 45.42 & 27.10 \\
~& Social Cognition and Knowledge Integration & Acc & \textbf{62.78} & 62.15 & - & 31.23 & 23.03 \\
~& Narrative and Structural Understanding & Acc &  55.17 & \textbf{59.48} & - & 25.86 & 25.00 \\
~& Professional Filming and Editing Techniques & Acc & \textbf{60.74} & 50.31 & - & 30.06 & 23.93 \\
\hline
~& Overall & Acc & 64.25 & \textbf{64.50} & - & 33.86 & 27.92 \\
\bottomrule[1.2pt]
\end{tabular}
%}
\caption{
Evaluation results on the VUE-CHAR benchmark, reporting temporal intersection-over-union (tIoU), spatial intersection-over-union (sIoU) and ASR errors in the \textit{Character} and question accuracy in the \textit{Reasoning} track.}
\label{tab:plot_results_t}
\end{table}


==> sections/tables/plot_performance_v2.tex <==
\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l| l| c | c c c c c}
\toprule[1.2pt]
%\multirow{3}{*}{Track} & \multirow{3}{*}{Category} & \multirow{2}{*}{Metric(\%)} 
\multirow{3}{*}{Track} & \multirow{3}{*}{Category} & \multirow{3}{*}{\shortstack{Metric\\(\%)}}
& \multicolumn{5}{c}{Models} \\
\cline{4-8}
~ & ~ & ~ 
& \shortstack{\textbf{Vidi}\\\textbf{2.5}}
& \shortstack{Gemini\\3 Pro.}
& \shortstack{GPT\\5}
& \shortstack{Qwen3\\VL}
& \shortstack{Qwen3\\Omni} \\
\hline

\multirow{3}{*}{Char.} & \multirow{3}{*}{-} ~ & tIoU & \textbf{71.74} & 66.04 & - & - & 49.31 \\
~ & ~ & sIoU & \textbf{60.31} & 12.99 & - & - & 7.74 \\
~ & ~ & WER $\downarrow$ & \textbf{23.15} & 28.20 & - & - & 56.36 \\

\hline\hline
\multirow{5}{*}{Rea.} 
~ & Perception and Understanding & Acc  & 66.25 & \textbf{80.42} & - & 35.00 & 40.83 \\
~ & Speech, Audio, and Sound Effect Reasoning & Acc & \textbf{74.43} & 66.03 & - & 45.42 & 27.10 \\
~ & Social Cognition and Knowledge Integration & Acc & \textbf{62.78} & 62.15 & - & 31.23 & 23.03 \\
~ & Narrative and Structural Understanding & Acc & 55.17 & \textbf{59.48} & - & 25.86 & 25.00 \\
~ & Professional Filming and Editing Techniques & Acc & \textbf{60.74} & 50.31 & - & 30.06 & 23.93 \\
\hline
~ & Overall & Acc & 64.25 & \textbf{64.50} & - & 33.86 & 27.92 \\
\bottomrule[1.2pt]
\end{tabular}}
\caption{
Evaluation results on the VUE-CHAR benchmark, reporting temporal intersection-over-union (tIoU), spatial intersection-over-union (sIoU) and ASR errors in the \textit{Character} (Char.) and question accuracy in the \textit{Reasoning} (Rea.) track.}
\label{tab:plot_results_t}
\end{table}

